Quantifying the effect of gate errors on variational quantum eigensolvers for quantum chemistry

Variational quantum eigensolvers (VQEs) are leading candidates to demonstrate near-term quantum advantage. Here, we conduct density-matrix simulations of leading gate-based VQEs for a range of molecules. We numerically quantify their level of tolerable depolarizing gate-errors. We find that: (i) The best-performing VQEs require gate-error probabilities between $10^{-6}$ and $10^{-4}$ ( $10^{-4}$ and $10^{-2}$ with error mitigation) to predict, within chemical accuracy, ground-state energies of small molecules with $4-14$ orbitals. (ii) ADAPT-VQEs that construct ansatz circuits iteratively outperform fixed-circuit VQEs. (iii) ADAPT-VQEs perform better with circuits constructed from gate-efficient rather than physically-motivated elements. (iv) The maximally-allowed gate-error probability, $p_c$, for any VQE to achieve chemical accuracy decreases with the number $\ncx$ of noisy two-qubit gates as $p_c\approxprop\ncx^{-1}$. Additionally, $p_c$ decreases with system size, even with error mitigation, implying that larger molecules require even lower gate-errors. Thus, quantum advantage via gate-based VQEs is unlikely unless gate-error probabilities are decreased by orders of magnitude.

==> Tables/table1.tex <==
\begin{table*}[t!]
    \def\arraystretch{1.5}
    %\setlength\tabcolsep{4pt} % default value: 6pt
    \begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}l*{11}{c}}
    \toprule
      \multicolumn{1}{c}{Molecule (Separation)}     &
      \multicolumn{1}{|l}{$\mathrm{H}_2$}           &
      \multicolumn{1}{l}{$\mathrm{H}_4$ (1\AA)}     &
      \multicolumn{1}{l}{$\mathrm{H}_4$ (3\AA)}     &
      \multicolumn{1}{l}{$\mathrm{LiH}$}            &
      \multicolumn{1}{l}{$\mathrm{HF}$}             &
      \multicolumn{1}{l|}{$\mathrm{BeH}_{2}$}       &
      \multicolumn{1}{|l}{$\mathrm{H}_4$ (1\AA)}    &
      \multicolumn{1}{l}{$\mathrm{H}_4$ (3\AA)}     &
      \multicolumn{1}{l|}{$\mathrm{LiH}$}           &
      \multicolumn{1}{|l}{$\mathrm{H}_2\mathrm{O}$} & 
      \multicolumn{1}{l}{$\mathrm{NH}_2^{-}$}
    \\
    \hline
      \multicolumn{1}{l}{{\parbox{5cm}{\color[HTML]{FE6100} Fermionic-ADAPT-VQE}}} &
      \multicolumn{1}{|r}{\num{5.30}}       &
      \multicolumn{1}{l}{\num{0.30}} &
      \multicolumn{1}{l}{\num{0.36}}             &
      \multicolumn{1}{l}{\num{0.52}}         &
      \multicolumn{1}{l}{\num{0.19}}    &
      \multicolumn{1}{l|}{\num{0.11}}                & 
      \multicolumn{1}{|l}{\num{0.30}}             &
      \multicolumn{1}{l}{\num{0.39}}     &
      \multicolumn{1}{l|}{\num{0.96}}  &  
      \multicolumn{1}{|l}{\num{0.04}}&
      \multicolumn{1}{l}{0.06}
    \\
      \multicolumn{1}{l}{{\parbox{5cm}{\color[HTML]{FE6100} Efficient fermionic-ADAPT-VQE}}} &
      \multicolumn{1}{|r}{\num{5.30}}       &
      \multicolumn{1}{l}{\num{1.38}}           &
      \multicolumn{1}{l}{\num{1.34}}        &
      \multicolumn{1}{l}{\num{2.02}}         &
      \multicolumn{1}{l}{\num{0.89}}    &
      \multicolumn{1}{l|}{\num{0.49}}                & 
      \multicolumn{1}{|l}{\num{1.51}}             &
      \multicolumn{1}{l}{\num{1.52}}     &
      \multicolumn{1}{l|}{\num{3.47}}  &
      \multicolumn{1}{|l}{ } &
      \multicolumn{1}{l}{ }
    \\
      \multicolumn{1}{l}{{\parbox{5cm}{\color[HTML]{64A5FF} QEB-ADAPT-VQE (Energy)}}} &
      \multicolumn{1}{|r}{\num{23.59}}      & 
      \multicolumn{1}{l}{\num{1.58}}           &
      \multicolumn{1}{l}{\num{1.05}}        &
      \multicolumn{1}{l}{\num{4.14}}         & 
      \multicolumn{1}{l}{\num{4.15}}     &
      \multicolumn{1}{l|}{\num{0.68}}                &
      \multicolumn{1}{|l}{\num{1.72}}             & 
      \multicolumn{1}{l}{\num{2.53}}             &
      \multicolumn{1}{l|}{\num{7.69}}     & 
      \multicolumn{1}{|l}{\num{0.35}}&
      \multicolumn{1}{l}{ }
    \\
      \multicolumn{1}{l}{{\parbox{5cm}{\color[HTML]{64A5FF} QEB-ADAPT-VQE (Gradient)}}}     & \multicolumn{1}{|r}{\num{23.59}}      & 
      \multicolumn{1}{l}{\num{1.73}}           &
      \multicolumn{1}{l}{\num{1.45}}            &
      \multicolumn{1}{l}{\num{2.25}}         & 
      \multicolumn{1}{l}{\num{0.97}}         &
      \multicolumn{1}{l|}{\num{0.59}}                &
      \multicolumn{1}{|l}{\num{1.73}}             &
      \multicolumn{1}{l}{\num{1.64}}             &
      \multicolumn{1}{l|}{\num{3.92}}  &
      \multicolumn{1}{|l}{\num{0.32}} &
      \multicolumn{1}{l}{ }
    \\
      \multicolumn{1}{l}{{\parbox{5cm}{\color[HTML]{76CCA4} qubit-ADAPT-VQE}}}               & \multicolumn{1}{|r}{\num{41.20}}      & 
      \multicolumn{1}{l}{\num{2.19}}           &
      \multicolumn{1}{l}{N/A}                   &
      \multicolumn{1}{l}{\num{4.28}}         &
      \multicolumn{1}{l}{\num{2.15}}         &
      \multicolumn{1}{l|}{\num{0.75}}                &
      \multicolumn{1}{|l}{\num{2.23}}             &
      \multicolumn{1}{l}{N/A}                   &
      \multicolumn{1}{l|}{\num{8.66}} &
      \multicolumn{1}{|l}{\num{0.30}} &
      \multicolumn{1}{l}{ }
    \\
    \botrule
    \end{tabular*}
    \caption{Maximum gate-error probabilities $p_{\mathrm{c}}$ [$\times10^{-5}$] for 
  which chemical accuracy is achieved.
  %
  The first set of columns presents data from Fig.~\ref{fig:1DPlots}, Sec.~\ref{1DPlotsSection}.
  %
  The second set of columns presents data from the top row of Fig.~\ref{fig:3DPlots}, Sec.~\ref{3DPlotsSection}.
  %
  The third set of data is derived using noise susceptibility, in Sec.~\ref{sec:scaling}.
  %
  \label{1DErrorTable}}
  \end{table*}
